Path Imputation Strategies for Signature Models of Irregular Time Series

The signature transform is a 'universal nonlinearity' on the space of continuous vector-valued paths, and has received attention for use in machine learning on time series. However, real-world temporal data is typically observed at discrete points in time, and must first be transformed into a continuous path before signature techniques can be applied. We make this step explicit by characterising it as an imputation problem, and empirically assess the impact of various imputation strategies when applying signature-based neural nets to irregular time series data. For one of these strategies, Gaussian process (GP) adapters, we propose an extension~(GP-PoM) that makes uncertainty information directly available to the subsequent classifier while at the same time preventing costly Monte-Carlo (MC) sampling. In our experiments, we find that the choice of imputation drastically affects shallow signature models, whereas deeper architectures are more robust. Next, we observe that uncertainty-aware predictions (based on GP-PoM or indicator imputations) are beneficial for predictive performance, even compared to the uncertainty-aware training of conventional GP adapters. In conclusion, we have demonstrated that the path construction is indeed crucial for signature models and that our proposed strategy leads to competitive performance in general, while improving robustness of signature models in particular.

==> tables/CharacterTrajectories.tex <==
\begin{tabular}{lllll}
\toprule
       & metric &                               w-AUROC &                                   BAC &                              Accuracy \\
subsampling & model &                                       &                                       &                                       \\
\midrule
Label-based & GP-DeepSig &                           $ 0.99852 $ &                           $ 0.93516 $ &                           $ 0.93273 $ \\
       & GP-DeepSig (PoM) &                           $ 0.99956 $ &                           $ 0.97529 $ &                           $ 0.97772 $ \\
       & GP-RNN &                           $ 0.99937 $ &                           $ 0.96977 $ &                           $ 0.97208 $ \\
       & GP-RNN (PoM) &               $  \mathbf{ 0.99993 } $ &            $  \underline{ 0.98933 } $ &            $  \underline{ 0.98955 } $ \\
       & GP-RNNSig &                           $ 0.98492 $ &                           $ 0.76234 $ &                           $ 0.77019 $ \\
       & GP-RNNSig (PoM) &                           $ 0.99706 $ &                           $ 0.94428 $ &                           $ 0.94708 $ \\
       & GP-Sig &                           $ 0.97624 $ &                           $ 0.73415 $ &                           $ 0.74088 $ \\
       & GP-Sig (PoM) &                           $ 0.99626 $ &                           $ 0.90547 $ &                           $ 0.90877 $ \\
       & causal-DeepSig &                            $ 0.9991 $ &                             $ 0.975 $ &                           $ 0.97632 $ \\
       & causal-RNN &                           $ 0.99935 $ &                            $ 0.9635 $ &                           $ 0.96657 $ \\
       & causal-RNNSig &                           $ 0.99447 $ &                           $ 0.88209 $ &                           $ 0.88997 $ \\
       & causal-Sig &                           $ 0.97949 $ &                           $ 0.75866 $ &                           $ 0.77577 $ \\
       & ff-DeepSig &                           $ 0.99992 $ &                           $ 0.97304 $ &                           $ 0.97563 $ \\
       & ff-RNN &                           $ 0.99967 $ &                           $ 0.98205 $ &                           $ 0.98329 $ \\
       & ff-RNNSig &                           $ 0.99816 $ &                           $ 0.93907 $ &                           $ 0.94359 $ \\
       & ff-Sig &                           $ 0.98022 $ &                           $ 0.77447 $ &                            $ 0.7883 $ \\
       & ind-DeepSig &  $  \mathbf{ \underline{ 0.99995 }} $ &               $  \mathbf{ 0.99012 } $ &               $  \mathbf{ 0.99095 } $ \\
       & ind-RNN &                            $ 0.9998 $ &                            $ 0.9856 $ &                           $ 0.98677 $ \\
       & ind-RNNSig &                           $ 0.99769 $ &                            $ 0.9331 $ &                           $ 0.93802 $ \\
       & ind-Sig &                           $ 0.97107 $ &                           $ 0.70657 $ &                           $ 0.72493 $ \\
       & lin-DeepSig &            $  \underline{ 0.99992 } $ &  $  \mathbf{ \underline{ 0.99079 }} $ &  $  \mathbf{ \underline{ 0.99164 }} $ \\
       & lin-RNN &                           $ 0.99935 $ &                           $ 0.97851 $ &                           $ 0.97981 $ \\
       & lin-RNNSig &                           $ 0.99883 $ &                           $ 0.95808 $ &                           $ 0.96031 $ \\
       & lin-Sig &                           $ 0.96044 $ &                           $ 0.66423 $ &                           $ 0.68454 $ \\
       & zero-DeepSig &                           $ 0.99977 $ &                           $ 0.97642 $ &                           $ 0.97841 $ \\
       & zero-RNN &                           $ 0.99963 $ &                           $ 0.97526 $ &                           $ 0.97702 $ \\
       & zero-RNNSig &                           $ 0.99798 $ &                           $ 0.92753 $ &                           $ 0.93315 $ \\
       & zero-Sig &                           $ 0.96446 $ &                            $ 0.6674 $ &                            $ 0.6915 $ \\
Random & GP-DeepSig &                           $ 0.98379 $ &                           $ 0.92496 $ &                           $ 0.91929 $ \\
       & GP-DeepSig (PoM) &            $  \underline{ 0.99984 } $ &                           $ 0.97822 $ &                           $ 0.97632 $ \\
       & GP-RNN &                           $ 0.99951 $ &                           $ 0.96926 $ &                           $ 0.97089 $ \\
       & GP-RNN (PoM) &                           $ 0.99984 $ &                           $ 0.98235 $ &                           $ 0.98329 $ \\
       & GP-RNNSig &                           $ 0.99529 $ &                           $ 0.89477 $ &                           $ 0.89903 $ \\
       & GP-RNNSig (PoM) &                           $ 0.99735 $ &                           $ 0.93434 $ &                           $ 0.94011 $ \\
       & GP-Sig &                           $ 0.97561 $ &                           $ 0.74296 $ &                           $ 0.75084 $ \\
       & GP-Sig (PoM) &                           $ 0.99547 $ &                           $ 0.91209 $ &                           $ 0.91435 $ \\
       & causal-DeepSig &                           $ 0.99976 $ &                           $ 0.98107 $ &                           $ 0.98259 $ \\
       & causal-RNN &                           $ 0.99965 $ &                           $ 0.97124 $ &                           $ 0.97354 $ \\
       & causal-RNNSig &                            $ 0.9982 $ &                           $ 0.93627 $ &                            $ 0.9415 $ \\
       & causal-Sig &                           $ 0.97171 $ &                           $ 0.68114 $ &                           $ 0.69568 $ \\
       & ff-DeepSig &                           $ 0.99979 $ &                           $ 0.98274 $ &                           $ 0.98398 $ \\
       & ff-RNN &                           $ 0.99912 $ &                           $ 0.97048 $ &                           $ 0.97284 $ \\
       & ff-RNNSig &                           $ 0.99867 $ &                            $ 0.9486 $ &                           $ 0.95265 $ \\
       & ff-Sig &                           $ 0.93721 $ &                           $ 0.56971 $ &                           $ 0.59471 $ \\
       & ind-DeepSig &                           $ 0.99916 $ &             $  \underline{ 0.9857 } $ &            $  \underline{ 0.98677 } $ \\
       & ind-RNN &                           $ 0.99962 $ &                           $ 0.97284 $ &                           $ 0.97493 $ \\
       & ind-RNNSig &                           $ 0.99843 $ &                           $ 0.94749 $ &                           $ 0.95125 $ \\
       & ind-Sig &                           $ 0.97142 $ &                           $ 0.70333 $ &                           $ 0.72632 $ \\
       & lin-DeepSig &  $  \mathbf{ \underline{ 0.99996 }} $ &  $  \mathbf{ \underline{ 0.99144 }} $ &  $  \mathbf{ \underline{ 0.99234 }} $ \\
       & lin-RNN &                           $ 0.99968 $ &                            $ 0.9761 $ &                           $ 0.97772 $ \\
       & lin-RNNSig &                           $ 0.99798 $ &                            $ 0.9368 $ &                            $ 0.9415 $ \\
       & lin-Sig &                           $ 0.89326 $ &                           $ 0.48317 $ &                           $ 0.50766 $ \\
       & zero-DeepSig &               $  \mathbf{ 0.99988 } $ &               $  \mathbf{ 0.98762 } $ &               $  \mathbf{ 0.98886 } $ \\
       & zero-RNN &                           $ 0.99927 $ &                           $ 0.96925 $ &                           $ 0.97145 $ \\
       & zero-RNNSig &                           $ 0.99763 $ &                           $ 0.92635 $ &                           $ 0.93175 $ \\
       & zero-Sig &                           $ 0.92155 $ &                           $ 0.44909 $ &                           $ 0.47563 $ \\
\bottomrule
\end{tabular}


==> tables/LSST.tex <==
\begin{tabular}{lllll}
\toprule
       & metric &                               w-AUROC &                                   BAC &                             Accuracy \\
subsampling & model &                                       &                                       &                                      \\
\midrule
Label-based & GP-DeepSig &                           $ 0.63585 $ &                           $ 0.18197 $ &                          $ 0.21999 $ \\
       & GP-DeepSig (PoM) &                           $ 0.74772 $ &                           $ 0.15754 $ &                           $ 0.1326 $ \\
       & GP-RNN &                            $ 0.6751 $ &                           $ 0.17692 $ &                          $ 0.34071 $ \\
       & GP-RNN (PoM) &            $  \underline{ 0.90377 } $ &                           $ 0.39123 $ &                          $ 0.46472 $ \\
       & GP-RNNSig &                           $ 0.60471 $ &                           $ 0.15081 $ &                          $ 0.33479 $ \\
       & GP-RNNSig (PoM) &                           $ 0.82478 $ &                           $ 0.28931 $ &                          $ 0.30089 $ \\
       & GP-Sig &                           $ 0.57096 $ &                            $ 0.1343 $ &                          $ 0.23946 $ \\
       & GP-Sig (PoM) &                           $ 0.59807 $ &                           $ 0.16114 $ &                         $ 0.095702 $ \\
       & causal-DeepSig &                           $ 0.80577 $ &                            $ 0.3125 $ &                          $ 0.48459 $ \\
       & causal-RNN &                           $ 0.84624 $ &                           $ 0.33731 $ &                          $ 0.53082 $ \\
       & causal-RNNSig &                           $ 0.82314 $ &                           $ 0.32955 $ &                          $ 0.51338 $ \\
       & causal-Sig &                           $ 0.59027 $ &                           $ 0.13125 $ &                          $ 0.33536 $ \\
       & ff-DeepSig &                           $ 0.75571 $ &                            $ 0.2625 $ &                          $ 0.34712 $ \\
       & ff-RNN &                           $ 0.84691 $ &                           $ 0.38555 $ &                          $ 0.53569 $ \\
       & ff-RNNSig &                           $ 0.82531 $ &                           $ 0.35215 $ &                          $ 0.48418 $ \\
       & ff-Sig &                           $ 0.63727 $ &                           $ 0.14316 $ &                           $ 0.3459 $ \\
       & ind-DeepSig &               $  \mathbf{ 0.95327 } $ &               $  \mathbf{ 0.51621 } $ &              $  \mathbf{ 0.80535 } $ \\
       & ind-RNN &  $  \mathbf{ \underline{ 0.98128 }} $ &  $  \mathbf{ \underline{ 0.59382 }} $ &  $  \mathbf{ \underline{ 0.8232 }} $ \\
       & ind-RNNSig &                           $ 0.81609 $ &                           $ 0.31671 $ &                          $ 0.41403 $ \\
       & ind-Sig &                           $ 0.57659 $ &                           $ 0.12875 $ &                          $ 0.33901 $ \\
       & lin-DeepSig &                           $ 0.76319 $ &                           $ 0.27597 $ &                          $ 0.46067 $ \\
       & lin-RNN &                           $ 0.84534 $ &                           $ 0.37092 $ &                          $ 0.53893 $ \\
       & lin-RNNSig &                           $ 0.83496 $ &                           $ 0.34416 $ &                          $ 0.52555 $ \\
       & lin-Sig &                           $ 0.66955 $ &                           $ 0.17077 $ &                          $ 0.36253 $ \\
       & zero-DeepSig &                           $ 0.74004 $ &                           $ 0.23683 $ &                          $ 0.33171 $ \\
       & zero-RNN &                           $ 0.89525 $ &            $  \underline{ 0.40892 } $ &           $  \underline{ 0.54663 } $ \\
       & zero-RNNSig &                           $ 0.78403 $ &                           $ 0.31934 $ &                          $ 0.46513 $ \\
       & zero-Sig &                            $ 0.5493 $ &                           $ 0.15275 $ &                          $ 0.30616 $ \\
Random & GP-DeepSig &                           $ 0.62195 $ &                           $ 0.15651 $ &                          $ 0.34643 $ \\
       & GP-DeepSig (PoM) &                           $ 0.74952 $ &                           $ 0.29438 $ &                          $ 0.36537 $ \\
       & GP-RNN &                           $ 0.64693 $ &                            $ 0.1847 $ &                          $ 0.35223 $ \\
       & GP-RNN (PoM) &                           $ 0.82287 $ &                           $ 0.36185 $ &                            $ 0.515 $ \\
       & GP-RNNSig &                           $ 0.60061 $ &                           $ 0.18232 $ &                          $ 0.33755 $ \\
       & GP-RNNSig (PoM) &                           $ 0.77488 $ &                           $ 0.27175 $ &                          $ 0.43674 $ \\
       & GP-Sig &                           $ 0.58776 $ &                            $ 0.1462 $ &                          $ 0.33228 $ \\
       & GP-Sig (PoM) &                            $ 0.5963 $ &                           $ 0.12667 $ &                          $ 0.35036 $ \\
       & causal-DeepSig &                           $ 0.77341 $ &                           $ 0.26873 $ &                          $ 0.32157 $ \\
       & causal-RNN &  $  \mathbf{ \underline{ 0.84593 }} $ &            $  \underline{ 0.37103 } $ &  $  \mathbf{ \underline{ 0.5661 }} $ \\
       & causal-RNNSig &                           $ 0.80265 $ &  $  \mathbf{ \underline{ 0.38461 }} $ &                          $ 0.50527 $ \\
       & causal-Sig &                           $ 0.55507 $ &                           $ 0.16425 $ &                          $ 0.33049 $ \\
       & ff-DeepSig &                           $ 0.75865 $ &                           $ 0.26642 $ &                          $ 0.26237 $ \\
       & ff-RNN &                 $  \mathbf{ 0.841 } $ &               $  \mathbf{ 0.37914 } $ &              $  \mathbf{ 0.55191 } $ \\
       & ff-RNNSig &                           $ 0.82349 $ &                           $ 0.35866 $ &                          $ 0.49635 $ \\
       & ff-Sig &                           $ 0.56967 $ &                           $ 0.12029 $ &                          $ 0.33901 $ \\
       & ind-DeepSig &                           $ 0.64712 $ &                           $ 0.17605 $ &                          $ 0.34347 $ \\
       & ind-RNN &                           $ 0.79579 $ &                           $ 0.31312 $ &                          $ 0.46634 $ \\
       & ind-RNNSig &                           $ 0.64653 $ &                           $ 0.18762 $ &                          $ 0.30616 $ \\
       & ind-Sig &                           $ 0.52971 $ &                           $ 0.11215 $ &                          $ 0.32036 $ \\
       & lin-DeepSig &                           $ 0.78331 $ &                           $ 0.25471 $ &                          $ 0.43512 $ \\
       & lin-RNN &            $  \underline{ 0.83925 } $ &                           $ 0.36831 $ &           $  \underline{ 0.54745 } $ \\
       & lin-RNNSig &                           $ 0.82926 $ &                           $ 0.31372 $ &                          $ 0.51135 $ \\
       & lin-Sig &                           $ 0.66071 $ &                           $ 0.18364 $ &                          $ 0.37713 $ \\
       & zero-DeepSig &                           $ 0.73129 $ &                           $ 0.20532 $ &                            $ 0.412 $ \\
       & zero-RNN &                            $ 0.8197 $ &                           $ 0.33041 $ &                           $ 0.5219 $ \\
       & zero-RNNSig &                           $ 0.78279 $ &                           $ 0.32638 $ &                          $ 0.45904 $ \\
       & zero-Sig &                           $ 0.54915 $ &                           $ 0.15811 $ &                         $ 0.076237 $ \\
\bottomrule
\end{tabular}


==> tables/PenDigits.tex <==
\begin{tabular}{lllll}
\toprule
       & metric &                               w-AUROC &                                   BAC &                              Accuracy \\
subsampling & model &                                       &                                       &                                       \\
\midrule
Label-based & GP-DeepSig &                           $ 0.88296 $ &                           $ 0.49497 $ &                           $ 0.49434 $ \\
       & GP-DeepSig (PoM) &            $  \underline{ 0.99933 } $ &            $  \underline{ 0.97306 } $ &            $  \underline{ 0.97313 } $ \\
       & GP-RNN &                           $ 0.90424 $ &                           $ 0.54095 $ &                           $ 0.53979 $ \\
       & GP-RNN (PoM) &                           $ 0.99899 $ &                           $ 0.96359 $ &                           $ 0.96341 $ \\
       & GP-RNNSig &                           $ 0.85031 $ &                           $ 0.43521 $ &                           $ 0.43436 $ \\
       & GP-RNNSig (PoM) &                           $ 0.99707 $ &                           $ 0.93331 $ &                           $ 0.93282 $ \\
       & GP-Sig &                           $ 0.81601 $ &                           $ 0.39828 $ &                           $ 0.39863 $ \\
       & GP-Sig (PoM) &                           $ 0.99148 $ &                           $ 0.88778 $ &                           $ 0.88708 $ \\
       & causal-DeepSig &                           $ 0.99308 $ &                           $ 0.89909 $ &                           $ 0.89794 $ \\
       & causal-RNN &                           $ 0.99255 $ &                           $ 0.89727 $ &                           $ 0.89651 $ \\
       & causal-RNNSig &                           $ 0.99308 $ &                           $ 0.88905 $ &                           $ 0.88822 $ \\
       & causal-Sig &                           $ 0.98389 $ &                           $ 0.83694 $ &                           $ 0.83591 $ \\
       & ff-DeepSig &                           $ 0.98934 $ &                           $ 0.89039 $ &                           $ 0.88908 $ \\
       & ff-RNN &                            $ 0.9933 $ &                           $ 0.90463 $ &                           $ 0.90395 $ \\
       & ff-RNNSig &                           $ 0.99351 $ &                           $ 0.89911 $ &                            $ 0.8988 $ \\
       & ff-Sig &                           $ 0.98248 $ &                           $ 0.83489 $ &                           $ 0.83362 $ \\
       & ind-DeepSig &               $  \mathbf{ 0.99941 } $ &  $  \mathbf{ \underline{ 0.97713 }} $ &  $  \mathbf{ \underline{ 0.97684 }} $ \\
       & ind-RNN &  $  \mathbf{ \underline{ 0.99951 }} $ &               $  \mathbf{ 0.97369 } $ &                $  \mathbf{ 0.9737 } $ \\
       & ind-RNNSig &                           $ 0.99732 $ &                           $ 0.92969 $ &                            $ 0.9291 $ \\
       & ind-Sig &                           $ 0.99325 $ &                           $ 0.89804 $ &                           $ 0.89737 $ \\
       & lin-DeepSig &                           $ 0.99567 $ &                           $ 0.92518 $ &                           $ 0.92424 $ \\
       & lin-RNN &                           $ 0.99539 $ &                           $ 0.92628 $ &                           $ 0.92567 $ \\
       & lin-RNNSig &                           $ 0.99495 $ &                           $ 0.90451 $ &                           $ 0.90366 $ \\
       & lin-Sig &                           $ 0.99041 $ &                           $ 0.87628 $ &                           $ 0.87479 $ \\
       & zero-DeepSig &                           $ 0.99274 $ &                           $ 0.90518 $ &                           $ 0.90395 $ \\
       & zero-RNN &                           $ 0.99586 $ &                           $ 0.92182 $ &                            $ 0.9211 $ \\
       & zero-RNNSig &                           $ 0.99326 $ &                            $ 0.8939 $ &                           $ 0.89308 $ \\
       & zero-Sig &                           $ 0.98303 $ &                           $ 0.83421 $ &                           $ 0.83305 $ \\
Random & GP-DeepSig &                           $ 0.90964 $ &                           $ 0.55605 $ &                           $ 0.55563 $ \\
       & GP-DeepSig (PoM) &                           $ 0.99527 $ &                           $ 0.92081 $ &                           $ 0.92024 $ \\
       & GP-RNN &                           $ 0.90783 $ &                           $ 0.54607 $ &                           $ 0.54594 $ \\
       & GP-RNN (PoM) &                           $ 0.99578 $ &            $  \underline{ 0.92919 } $ &            $  \underline{ 0.92853 } $ \\
       & GP-RNNSig &                           $ 0.86954 $ &                           $ 0.47817 $ &                           $ 0.47802 $ \\
       & GP-RNNSig (PoM) &                           $ 0.99336 $ &                            $ 0.9066 $ &                           $ 0.90595 $ \\
       & GP-Sig &                           $ 0.84778 $ &                           $ 0.44101 $ &                             $ 0.442 $ \\
       & GP-Sig (PoM) &                           $ 0.98924 $ &                           $ 0.87698 $ &                           $ 0.87679 $ \\
       & causal-DeepSig &                           $ 0.99262 $ &                           $ 0.89371 $ &                           $ 0.89308 $ \\
       & causal-RNN &                            $ 0.9925 $ &                           $ 0.89175 $ &                           $ 0.89165 $ \\
       & causal-RNNSig &                           $ 0.99115 $ &                           $ 0.88842 $ &                           $ 0.88794 $ \\
       & causal-Sig &                           $ 0.98249 $ &                           $ 0.82081 $ &                            $ 0.8199 $ \\
       & ff-DeepSig &                           $ 0.99055 $ &                           $ 0.88501 $ &                           $ 0.88451 $ \\
       & ff-RNN &                           $ 0.99419 $ &                           $ 0.90398 $ &                           $ 0.90337 $ \\
       & ff-RNNSig &                            $ 0.9922 $ &                           $ 0.88938 $ &                           $ 0.88908 $ \\
       & ff-Sig &                           $ 0.98571 $ &                           $ 0.84269 $ &                           $ 0.84191 $ \\
       & ind-DeepSig &                $  \mathbf{ 0.9972 } $ &               $  \mathbf{ 0.93715 } $ &               $  \mathbf{ 0.93654 } $ \\
       & ind-RNN &  $  \mathbf{ \underline{ 0.99771 }} $ &  $  \mathbf{ \underline{ 0.94814 }} $ &  $  \mathbf{ \underline{ 0.94768 }} $ \\
       & ind-RNNSig &                           $ 0.99562 $ &                           $ 0.91775 $ &                            $ 0.9171 $ \\
       & ind-Sig &                           $ 0.98783 $ &                           $ 0.84821 $ &                           $ 0.84763 $ \\
       & lin-DeepSig &                           $ 0.99438 $ &                           $ 0.91783 $ &                           $ 0.91767 $ \\
       & lin-RNN &                           $ 0.99463 $ &                           $ 0.91445 $ &                           $ 0.91395 $ \\
       & lin-RNNSig &            $  \underline{ 0.99621 } $ &                           $ 0.92118 $ &                           $ 0.92081 $ \\
       & lin-Sig &                           $ 0.99149 $ &                            $ 0.8843 $ &                           $ 0.88393 $ \\
       & zero-DeepSig &                             $ 0.994 $ &                           $ 0.90535 $ &                           $ 0.90452 $ \\
       & zero-RNN &                            $ 0.9955 $ &                           $ 0.91814 $ &                           $ 0.91795 $ \\
       & zero-RNNSig &                           $ 0.99113 $ &                           $ 0.88433 $ &                           $ 0.88422 $ \\
       & zero-Sig &                           $ 0.98705 $ &                           $ 0.83734 $ &                           $ 0.83648 $ \\
\bottomrule
\end{tabular}


==> tables/Physionet2012.tex <==
\begin{tabular}{lll}
\toprule
metric &                                 AUROC &                     Average Precision \\
model            &                                       &                                       \\
\midrule
GP-DeepSig       &                           $ 0.83057 $ &                           $ 0.48053 $ \\
GP-DeepSig (PoM) &                            $ 0.8202 $ &                           $ 0.49333 $ \\
GP-RNN           &                           $ 0.82501 $ &                           $ 0.48862 $ \\
GP-RNN (PoM)     &                            $ 0.8411 $ &                           $ 0.50316 $ \\
GP-RNNSig        &                           $ 0.75912 $ &                           $ 0.36152 $ \\
GP-RNNSig (PoM)  &                           $ 0.77133 $ &                            $ 0.4031 $ \\
GP-Sig           &                           $ 0.73406 $ &                           $ 0.35228 $ \\
GP-Sig (PoM)     &                           $ 0.76132 $ &                           $ 0.34929 $ \\
causal-DeepSig   &                           $ 0.83786 $ &                           $ 0.49095 $ \\
causal-RNN       &               $  \mathbf{ 0.84687 } $ &               $  \mathbf{ 0.51729 } $ \\
causal-RNNSig    &                           $ 0.81896 $ &                           $ 0.46484 $ \\
causal-Sig       &                           $ 0.83908 $ &                           $ 0.48984 $ \\
ff-DeepSig       &                           $ 0.82189 $ &                           $ 0.48037 $ \\
ff-RNN           &            $  \underline{ 0.84655 } $ &  $  \mathbf{ \underline{ 0.52581 }} $ \\
ff-RNNSig        &                           $ 0.80963 $ &                           $ 0.43971 $ \\
ff-Sig           &                           $ 0.84356 $ &                            $ 0.5036 $ \\
ind-DeepSig      &                           $ 0.82432 $ &                           $ 0.48006 $ \\
ind-RNN          &  $  \mathbf{ \underline{ 0.84961 }} $ &            $  \underline{ 0.51611 } $ \\
ind-RNNSig       &                           $ 0.83766 $ &                           $ 0.50512 $ \\
ind-Sig          &                           $ 0.80753 $ &                           $ 0.46094 $ \\
lin-DeepSig      &                            $ 0.8338 $ &                           $ 0.49465 $ \\
lin-RNN          &                           $ 0.84303 $ &                           $ 0.51061 $ \\
lin-RNNSig       &                            $ 0.7769 $ &                           $ 0.42146 $ \\
lin-Sig          &                           $ 0.83442 $ &                           $ 0.49693 $ \\
zero-DeepSig     &                           $ 0.82405 $ &                           $ 0.47245 $ \\
zero-RNN         &                           $ 0.84041 $ &                           $ 0.49561 $ \\
zero-RNNSig      &                           $ 0.78151 $ &                           $ 0.41783 $ \\
zero-Sig         &                           $ 0.80593 $ &                           $ 0.44305 $ \\
\bottomrule
\end{tabular}


==> tables/repetitions_CharacterTrajectories.tex <==
\begin{tabular}{lllll}
\toprule
       & metric &                                          w-AUROC &                                             BAC &                                        Accuracy \\
subsampling & model &                                                  &                                                 &                                                 \\
\midrule
Label-based & GP-DeepSig &                             $ 0.9929 \pm 0.007 $ &                             $ 0.8955 \pm 0.03 $ &                            $ 0.8937 \pm 0.031 $ \\
       & GP-RNN &                           $ 0.9997 \pm 0.00011 $ &                           $ 0.9771 \pm 0.0027 $ &                           $ 0.9787 \pm 0.0025 $ \\
       & GP-RNNSig &                             $ 0.9667 \pm 0.024 $ &                             $ 0.6572 \pm 0.14 $ &                             $ 0.6705 \pm 0.13 $ \\
       & GP-Sig &                             $ 0.9528 \pm 0.016 $ &                            $ 0.6242 \pm 0.061 $ &                             $ 0.6361 \pm 0.06 $ \\
       & GP-PoM-DeepSig &                            $ 0.9958 \pm 0.0067 $ &                            $ 0.9516 \pm 0.015 $ &                            $ 0.9496 \pm 0.017 $ \\
       & GP-PoM-RNN &            $  \underline{ 0.9997 \pm 0.00015 } $ &               $  \mathbf{ 0.9816 \pm 0.0066 } $ &                $  \mathbf{ 0.9827 \pm 0.006 } $ \\
       & GP-PoM-RNNSig &                            $ 0.997 \pm 0.00089 $ &                            $ 0.9278 \pm 0.012 $ &                            $ 0.9323 \pm 0.011 $ \\
       & GP-PoM-Sig &                           $ 0.9952 \pm 0.00075 $ &                            $ 0.8863 \pm 0.014 $ &                            $ 0.8901 \pm 0.013 $ \\
       & causal-DeepSig &                           $ 0.9994 \pm 0.00024 $ &                           $ 0.9727 \pm 0.0071 $ &                           $ 0.9744 \pm 0.0062 $ \\
       & causal-RNN &                           $ 0.9996 \pm 9.8e-05 $ &                           $ 0.9724 \pm 0.0052 $ &                           $ 0.9741 \pm 0.0048 $ \\
       & causal-RNNSig &                            $ 0.9952 \pm 0.0016 $ &                            $ 0.8992 \pm 0.023 $ &                            $ 0.9058 \pm 0.022 $ \\
       & causal-Sig &                              $ 0.9575 \pm 0.05 $ &                             $ 0.6631 \pm 0.22 $ &                             $ 0.6826 \pm 0.21 $ \\
       & ff-DeepSig &                           $ 0.9995 \pm 0.00041 $ &                           $ 0.9796 \pm 0.0068 $ &                           $ 0.9808 \pm 0.0066 $ \\
       & ff-RNN &                           $ 0.9994 \pm 0.00011 $ &                           $ 0.9694 \pm 0.0049 $ &                           $ 0.9716 \pm 0.0044 $ \\
       & ff-RNNSig &                           $ 0.9972 \pm 0.00071 $ &                            $ 0.9257 \pm 0.011 $ &                             $ 0.9315 \pm 0.01 $ \\
       & ff-Sig &                             $ 0.9483 \pm 0.081 $ &                             $ 0.6717 \pm 0.26 $ &                             $ 0.6865 \pm 0.26 $ \\
       & ind-DeepSig &  $  \mathbf{ \underline{ 0.9999 \pm 0.00013 }} $ &  $  \mathbf{ \underline{ 0.9859 \pm 0.0029 }} $ &  $  \mathbf{ \underline{ 0.9872 \pm 0.0026 }} $ \\
       & ind-RNN &                            $ 0.9992 \pm 0.0002 $ &                           $ 0.9641 \pm 0.0041 $ &                           $ 0.9667 \pm 0.0037 $ \\
       & ind-RNNSig &                            $ 0.998 \pm 0.00032 $ &                           $ 0.9379 \pm 0.0046 $ &                           $ 0.9423 \pm 0.0044 $ \\
       & ind-Sig &                               $ 0.9166 \pm 0.1 $ &                             $ 0.5642 \pm 0.23 $ &                             $ 0.5838 \pm 0.23 $ \\
       & lin-DeepSig &                            $ 0.9997 \pm 0.0001 $ &            $  \underline{ 0.9805 \pm 0.0074 } $ &            $  \underline{ 0.9822 \pm 0.0067 } $ \\
       & lin-RNN &                           $ 0.9988 \pm 0.00059 $ &                            $ 0.9691 \pm 0.013 $ &                            $ 0.9712 \pm 0.012 $ \\
       & lin-RNNSig &                           $ 0.9988 \pm 0.00035 $ &                           $ 0.9485 \pm 0.0092 $ &                           $ 0.9529 \pm 0.0084 $ \\
       & lin-Sig &                              $ 0.8044 \pm 0.18 $ &                             $ 0.3119 \pm 0.24 $ &                             $ 0.3233 \pm 0.25 $ \\
       & zero-DeepSig &                $  \mathbf{ 0.9998 \pm 0.0001 } $ &                           $ 0.9803 \pm 0.0036 $ &                           $ 0.9819 \pm 0.0036 $ \\
       & zero-RNN &                           $ 0.9997 \pm 0.00014 $ &                           $ 0.9743 \pm 0.0057 $ &                            $ 0.9755 \pm 0.006 $ \\
       & zero-RNNSig &                             $ 0.997 \pm 0.0013 $ &                            $ 0.9175 \pm 0.018 $ &                            $ 0.9237 \pm 0.017 $ \\
       & zero-Sig &                              $ 0.7773 \pm 0.24 $ &                             $ 0.3799 \pm 0.34 $ &                             $ 0.3896 \pm 0.35 $ \\
Random & GP-DeepSig &                             $ 0.9899 \pm 0.011 $ &                            $ 0.9082 \pm 0.024 $ &                            $ 0.9047 \pm 0.023 $ \\
       & GP-RNN &                           $ 0.9991 \pm 0.00032 $ &                           $ 0.9628 \pm 0.0069 $ &                           $ 0.9649 \pm 0.0071 $ \\
       & GP-RNNSig &                            $ 0.994 \pm 0.00094 $ &                            $ 0.8759 \pm 0.021 $ &                             $ 0.8814 \pm 0.02 $ \\
       & GP-Sig &                             $ 0.9486 \pm 0.018 $ &                            $ 0.6128 \pm 0.064 $ &                            $ 0.6245 \pm 0.065 $ \\
       & GP-PoM-DeepSig &                             $ 0.997 \pm 0.0039 $ &                             $ 0.9401 \pm 0.05 $ &                            $ 0.9364 \pm 0.053 $ \\
       & GP-PoM-RNN &            $  \underline{ 0.9997 \pm 0.00011 } $ &                           $ 0.9801 \pm 0.0051 $ &                           $ 0.9811 \pm 0.0051 $ \\
       & GP-PoM-RNNSig &                           $ 0.9979 \pm 0.00074 $ &                           $ 0.9331 \pm 0.0096 $ &                            $ 0.9384 \pm 0.009 $ \\
       & GP-PoM-Sig &                           $ 0.9958 \pm 0.00031 $ &                           $ 0.8957 \pm 0.0094 $ &                           $ 0.8993 \pm 0.0091 $ \\
       & causal-DeepSig &                           $ 0.9996 \pm 0.00023 $ &                           $ 0.9777 \pm 0.0023 $ &                           $ 0.9795 \pm 0.0018 $ \\
       & causal-RNN &                           $ 0.9995 \pm 0.00023 $ &                           $ 0.9766 \pm 0.0072 $ &                           $ 0.9781 \pm 0.0068 $ \\
       & causal-RNNSig &                           $ 0.9981 \pm 0.00044 $ &                           $ 0.9327 \pm 0.0073 $ &                           $ 0.9375 \pm 0.0074 $ \\
       & causal-Sig &                            $ 0.9674 \pm 0.0058 $ &                            $ 0.7139 \pm 0.038 $ &                            $ 0.7325 \pm 0.036 $ \\
       & ff-DeepSig &                            $ 0.9996 \pm 0.0003 $ &                           $ 0.9797 \pm 0.0038 $ &                           $ 0.9812 \pm 0.0037 $ \\
       & ff-RNN &                            $ 0.9995 \pm 0.0001 $ &                           $ 0.9779 \pm 0.0031 $ &                           $ 0.9794 \pm 0.0028 $ \\
       & ff-RNNSig &                           $ 0.9984 \pm 0.00047 $ &                           $ 0.9411 \pm 0.0077 $ &                            $ 0.946 \pm 0.0074 $ \\
       & ff-Sig &                             $ 0.5431 \pm 0.042 $ &                            $ 0.07387 \pm 0.03 $ &                           $ 0.07117 \pm 0.024 $ \\
       & ind-DeepSig &                           $ 0.9996 \pm 0.00033 $ &                $  \mathbf{ 0.9863 \pm 0.005 } $ &               $  \mathbf{ 0.9873 \pm 0.0048 } $ \\
       & ind-RNN &                           $ 0.9995 \pm 0.00024 $ &                            $ 0.975 \pm 0.0053 $ &                            $ 0.9766 \pm 0.005 $ \\
       & ind-RNNSig &                           $ 0.9975 \pm 0.00078 $ &                            $ 0.9309 \pm 0.011 $ &                           $ 0.9364 \pm 0.0095 $ \\
       & ind-Sig &                              $ 0.6692 \pm 0.18 $ &                             $ 0.1848 \pm 0.19 $ &                             $ 0.1907 \pm 0.19 $ \\
       & lin-DeepSig &  $  \mathbf{ \underline{ 0.9998 \pm 6.8e-05 }} $ &   $  \mathbf{ \underline{ 0.989 \pm 0.0021 }} $ &     $  \mathbf{ \underline{ 0.99 \pm 0.002 }} $ \\
       & lin-RNN &                           $ 0.9993 \pm 0.00043 $ &                            $ 0.9767 \pm 0.009 $ &                            $ 0.9779 \pm 0.008 $ \\
       & lin-RNNSig &                           $ 0.9977 \pm 0.00037 $ &                           $ 0.9275 \pm 0.0066 $ &                           $ 0.9327 \pm 0.0066 $ \\
       & lin-Sig &                             $ 0.5502 \pm 0.067 $ &                           $ 0.09436 \pm 0.033 $ &                           $ 0.09958 \pm 0.041 $ \\
       & zero-DeepSig &               $  \mathbf{ 0.9998 \pm 0.00013 } $ &            $  \underline{ 0.9834 \pm 0.0064 } $ &            $  \underline{ 0.9845 \pm 0.0062 } $ \\
       & zero-RNN &                           $ 0.9989 \pm 0.00052 $ &                              $ 0.96 \pm 0.011 $ &                             $ 0.9625 \pm 0.01 $ \\
       & zero-RNNSig &                           $ 0.9968 \pm 0.00063 $ &                           $ 0.9215 \pm 0.0088 $ &                           $ 0.9274 \pm 0.0082 $ \\
       & zero-Sig &                              $ 0.97 \pm 0.0039 $ &                            $ 0.6996 \pm 0.042 $ &                              $ 0.717 \pm 0.04 $ \\
\bottomrule
\end{tabular}


==> tables/repetitions_LSST.tex <==
\begin{tabular}{lllll}
\toprule
       & metric &                                         w-AUROC &                                             BAC &                                       Accuracy \\
subsampling & model &                                                 &                                                 &                                                \\
\midrule
Label-based & GP-DeepSig &                            $ 0.5969 \pm 0.034 $ &                            $ 0.1314 \pm 0.039 $ &                           $ 0.2833 \pm 0.055 $ \\
       & GP-RNN &                            $ 0.6927 \pm 0.015 $ &                           $ 0.1656 \pm 0.0046 $ &                           $ 0.339 \pm 0.0036 $ \\
       & GP-RNNSig &                           $ 0.6003 \pm 0.0048 $ &                            $ 0.1678 \pm 0.016 $ &                          $ 0.3363 \pm 0.0021 $ \\
       & GP-Sig &                           $ 0.5738 \pm 0.0055 $ &                            $ 0.1406 \pm 0.012 $ &                           $ 0.2429 \pm 0.021 $ \\
       & GP-PoM-DeepSig &                            $ 0.6441 \pm 0.068 $ &                            $ 0.1386 \pm 0.024 $ &                          $ 0.08743 \pm 0.029 $ \\
       & GP-PoM-RNN &                            $ 0.8281 \pm 0.043 $ &                            $ 0.2948 \pm 0.071 $ &                            $ 0.2978 \pm 0.12 $ \\
       & GP-PoM-RNNSig &                            $ 0.8293 \pm 0.015 $ &                            $ 0.3175 \pm 0.023 $ &                           $ 0.3544 \pm 0.036 $ \\
       & GP-PoM-Sig &                            $ 0.5882 \pm 0.014 $ &                           $ 0.1378 \pm 0.0053 $ &                           $ 0.1019 \pm 0.014 $ \\
       & causal-DeepSig &                            $ 0.7534 \pm 0.035 $ &                            $ 0.2548 \pm 0.059 $ &                            $ 0.394 \pm 0.058 $ \\
       & causal-RNN &                           $ 0.8411 \pm 0.0061 $ &                            $ 0.3776 \pm 0.017 $ &                           $ 0.5301 \pm 0.017 $ \\
       & causal-RNNSig &                           $ 0.8234 \pm 0.0023 $ &                            $ 0.3357 \pm 0.028 $ &                          $ 0.5028 \pm 0.0097 $ \\
       & causal-Sig &                            $ 0.5884 \pm 0.032 $ &                            $ 0.1226 \pm 0.028 $ &                           $ 0.3416 \pm 0.013 $ \\
       & ff-DeepSig &                            $ 0.7776 \pm 0.026 $ &                            $ 0.2747 \pm 0.042 $ &                           $ 0.4224 \pm 0.054 $ \\
       & ff-RNN &                           $ 0.8415 \pm 0.0067 $ &                            $ 0.3862 \pm 0.016 $ &                          $ 0.5298 \pm 0.0067 $ \\
       & ff-RNNSig &                           $ 0.8243 \pm 0.0044 $ &                            $ 0.3408 \pm 0.014 $ &                          $ 0.5056 \pm 0.0068 $ \\
       & ff-Sig &                            $ 0.642 \pm 0.0081 $ &                            $ 0.1478 \pm 0.012 $ &                          $ 0.3526 \pm 0.0052 $ \\
       & ind-DeepSig &                 $  \mathbf{ 0.9535 \pm 0.01 } $ &                $  \mathbf{ 0.5212 \pm 0.021 } $ &               $  \mathbf{ 0.7728 \pm 0.022 } $ \\
       & ind-RNN &  $  \mathbf{ \underline{ 0.9813 \pm 0.0024 }} $ &   $  \mathbf{ \underline{ 0.6189 \pm 0.039 }} $ &  $  \mathbf{ \underline{ 0.8361 \pm 0.015 }} $ \\
       & ind-RNNSig &                            $ 0.8263 \pm 0.018 $ &                            $ 0.2912 \pm 0.031 $ &                           $ 0.4115 \pm 0.025 $ \\
       & ind-Sig &                           $ 0.5708 \pm 0.0086 $ &                           $ 0.1281 \pm 0.0095 $ &                           $ 0.3262 \pm 0.011 $ \\
       & lin-DeepSig &                            $ 0.7396 \pm 0.032 $ &                           $ 0.2136 \pm 0.0075 $ &                            $ 0.365 \pm 0.063 $ \\
       & lin-RNN &                            $ 0.8493 \pm 0.003 $ &                            $ 0.401 \pm 0.0097 $ &           $  \underline{ 0.5402 \pm 0.0082 } $ \\
       & lin-RNNSig &                            $ 0.8288 \pm 0.008 $ &                            $ 0.3255 \pm 0.013 $ &                           $ 0.4933 \pm 0.024 $ \\
       & lin-Sig &                            $ 0.6669 \pm 0.018 $ &                           $ 0.1734 \pm 0.0078 $ &                          $ 0.3573 \pm 0.0057 $ \\
       & zero-DeepSig &                            $ 0.7578 \pm 0.012 $ &                             $ 0.236 \pm 0.033 $ &                           $ 0.4202 \pm 0.017 $ \\
       & zero-RNN &            $  \underline{ 0.8791 \pm 0.0095 } $ &             $  \underline{ 0.4048 \pm 0.019 } $ &                           $ 0.5327 \pm 0.021 $ \\
       & zero-RNNSig &                            $ 0.7943 \pm 0.005 $ &                            $ 0.3438 \pm 0.012 $ &                          $ 0.4652 \pm 0.0045 $ \\
       & zero-Sig &                            $ 0.5297 \pm 0.011 $ &                            $ 0.1195 \pm 0.011 $ &                           $ 0.2853 \pm 0.084 $ \\
Random & GP-DeepSig &                           $ 0.6213 \pm 0.0096 $ &                            $ 0.1619 \pm 0.018 $ &                          $ 0.3432 \pm 0.0016 $ \\
       & GP-RNN &                             $ 0.6264 \pm 0.03 $ &                            $ 0.1736 \pm 0.022 $ &                           $ 0.3452 \pm 0.012 $ \\
       & GP-RNNSig &                            $ 0.6059 \pm 0.004 $ &                            $ 0.1714 \pm 0.015 $ &                          $ 0.3371 \pm 0.0065 $ \\
       & GP-Sig &                            $ 0.5798 \pm 0.013 $ &                            $ 0.1361 \pm 0.011 $ &                            $ 0.331 \pm 0.004 $ \\
       & GP-PoM-DeepSig &                            $ 0.7077 \pm 0.029 $ &                            $ 0.2182 \pm 0.027 $ &                           $ 0.4011 \pm 0.024 $ \\
       & GP-PoM-RNN &                           $ 0.8232 \pm 0.0083 $ &             $  \underline{ 0.3737 \pm 0.019 } $ &                           $ 0.5251 \pm 0.026 $ \\
       & GP-PoM-RNNSig &                            $ 0.7584 \pm 0.016 $ &                            $ 0.2668 \pm 0.019 $ &                           $ 0.4179 \pm 0.019 $ \\
       & GP-PoM-Sig &                            $ 0.588 \pm 0.0056 $ &                             $ 0.132 \pm 0.013 $ &                           $ 0.3461 \pm 0.008 $ \\
       & causal-DeepSig &                            $ 0.7427 \pm 0.021 $ &                            $ 0.2218 \pm 0.027 $ &                            $ 0.341 \pm 0.066 $ \\
       & causal-RNN &               $  \mathbf{ 0.8394 \pm 0.0073 } $ &                $  \mathbf{ 0.3741 \pm 0.023 } $ &  $  \mathbf{ \underline{ 0.5456 \pm 0.011 }} $ \\
       & causal-RNNSig &                             $ 0.7719 \pm 0.05 $ &                            $ 0.3168 \pm 0.055 $ &                            $ 0.464 \pm 0.053 $ \\
       & causal-Sig &                           $ 0.5268 \pm 0.0082 $ &                           $ 0.1163 \pm 0.0081 $ &                           $ 0.2603 \pm 0.099 $ \\
       & ff-DeepSig &                            $ 0.7876 \pm 0.012 $ &                            $ 0.2787 \pm 0.022 $ &                           $ 0.4685 \pm 0.014 $ \\
       & ff-RNN &  $  \mathbf{ \underline{ 0.8427 \pm 0.0057 }} $ &  $  \mathbf{ \underline{ 0.3832 \pm 0.0055 }} $ &            $  \underline{ 0.5324 \pm 0.013 } $ \\
       & ff-RNNSig &                           $ 0.8229 \pm 0.0035 $ &                            $ 0.3352 \pm 0.011 $ &                            $ 0.502 \pm 0.011 $ \\
       & ff-Sig &                            $ 0.5603 \pm 0.023 $ &                            $ 0.1298 \pm 0.015 $ &                            $ 0.2852 \pm 0.12 $ \\
       & ind-DeepSig &                            $ 0.6986 \pm 0.016 $ &                            $ 0.2081 \pm 0.012 $ &                             $ 0.364 \pm 0.04 $ \\
       & ind-RNN &                             $ 0.7696 \pm 0.03 $ &                            $ 0.2918 \pm 0.026 $ &                           $ 0.4218 \pm 0.044 $ \\
       & ind-RNNSig &                             $ 0.637 \pm 0.015 $ &                            $ 0.1837 \pm 0.016 $ &                           $ 0.3031 \pm 0.019 $ \\
       & ind-Sig &                            $ 0.5383 \pm 0.015 $ &                            $ 0.1221 \pm 0.023 $ &                          $ 0.3267 \pm 0.0036 $ \\
       & lin-DeepSig &                             $ 0.7516 \pm 0.04 $ &                            $ 0.2366 \pm 0.044 $ &                           $ 0.4032 \pm 0.054 $ \\
       & lin-RNN &            $  \underline{ 0.8378 \pm 0.0051 } $ &                            $ 0.3682 \pm 0.024 $ &              $  \mathbf{ 0.5344 \pm 0.0061 } $ \\
       & lin-RNNSig &                             $ 0.8159 \pm 0.01 $ &                             $ 0.2981 \pm 0.02 $ &                           $ 0.4929 \pm 0.016 $ \\
       & lin-Sig &                             $ 0.655 \pm 0.031 $ &                            $ 0.1711 \pm 0.035 $ &                          $ 0.3633 \pm 0.0098 $ \\
       & zero-DeepSig &                            $ 0.6951 \pm 0.049 $ &                            $ 0.1523 \pm 0.047 $ &                           $ 0.3527 \pm 0.041 $ \\
       & zero-RNN &                           $ 0.8174 \pm 0.0042 $ &                            $ 0.3558 \pm 0.027 $ &                           $ 0.5007 \pm 0.022 $ \\
       & zero-RNNSig &                            $ 0.776 \pm 0.0063 $ &                            $ 0.3129 \pm 0.016 $ &                           $ 0.4595 \pm 0.013 $ \\
       & zero-Sig &                             $ 0.529 \pm 0.015 $ &                            $ 0.1187 \pm 0.023 $ &                          $ 0.3261 \pm 0.0065 $ \\
\bottomrule
\end{tabular}


==> tables/repetitions_PenDigits.tex <==
\begin{tabular}{lllll}
\toprule
       & metric &                                          w-AUROC &                                             BAC &                                        Accuracy \\
subsampling & model &                                                  &                                                 &                                                 \\
\midrule
Label-based & GP-DeepSig &                             $ 0.9289 \pm 0.015 $ &                            $ 0.6059 \pm 0.041 $ &                            $ 0.6048 \pm 0.041 $ \\
       & GP-RNN &                             $ 0.9517 \pm 0.014 $ &                            $ 0.6754 \pm 0.048 $ &                            $ 0.6743 \pm 0.048 $ \\
       & GP-RNNSig &                              $ 0.845 \pm 0.013 $ &                             $ 0.4218 \pm 0.02 $ &                            $ 0.4214 \pm 0.019 $ \\
       & GP-Sig &                             $ 0.8031 \pm 0.027 $ &                            $ 0.3777 \pm 0.036 $ &                            $ 0.3772 \pm 0.036 $ \\
       & GP-PoM-DeepSig &            $  \underline{ 0.9993 \pm 0.00032 } $ &                 $  \mathbf{ 0.974 \pm 0.003 } $ &                $  \mathbf{ 0.9738 \pm 0.003 } $ \\
       & GP-PoM-RNN &                            $ 0.999 \pm 0.00016 $ &                            $ 0.9635 \pm 0.003 $ &                            $ 0.9631 \pm 0.003 $ \\
       & GP-PoM-RNNSig &                           $ 0.9967 \pm 0.00073 $ &                           $ 0.9302 \pm 0.0076 $ &                           $ 0.9297 \pm 0.0076 $ \\
       & GP-PoM-Sig &                            $ 0.9915 \pm 0.0014 $ &                            $ 0.8809 \pm 0.015 $ &                              $ 0.88 \pm 0.015 $ \\
       & causal-DeepSig &                           $ 0.9924 \pm 0.00075 $ &                           $ 0.8962 \pm 0.0075 $ &                           $ 0.8951 \pm 0.0075 $ \\
       & causal-RNN &                           $ 0.9924 \pm 0.00098 $ &                            $ 0.895 \pm 0.0048 $ &                            $ 0.8942 \pm 0.005 $ \\
       & causal-RNNSig &                            $ 0.993 \pm 0.00041 $ &                           $ 0.8919 \pm 0.0048 $ &                           $ 0.8914 \pm 0.0049 $ \\
       & causal-Sig &                           $ 0.9837 \pm 0.00065 $ &                             $ 0.832 \pm 0.004 $ &                           $ 0.8308 \pm 0.0043 $ \\
       & ff-DeepSig &                           $ 0.9901 \pm 0.00072 $ &                           $ 0.8821 \pm 0.0043 $ &                           $ 0.8809 \pm 0.0043 $ \\
       & ff-RNN &                           $ 0.9933 \pm 0.00046 $ &                           $ 0.8975 \pm 0.0041 $ &                           $ 0.8966 \pm 0.0042 $ \\
       & ff-RNNSig &                           $ 0.9927 \pm 0.00015 $ &                           $ 0.8979 \pm 0.0038 $ &                           $ 0.8974 \pm 0.0039 $ \\
       & ff-Sig &                           $ 0.9831 \pm 0.00045 $ &                           $ 0.8374 \pm 0.0042 $ &                            $ 0.8362 \pm 0.004 $ \\
       & ind-DeepSig &  $  \mathbf{ \underline{ 0.9996 \pm 0.00013 }} $ &  $  \mathbf{ \underline{ 0.9807 \pm 0.0018 }} $ &  $  \mathbf{ \underline{ 0.9806 \pm 0.0019 }} $ \\
       & ind-RNN &               $  \mathbf{ 0.9996 \pm 9.2e-05 } $ &            $  \underline{ 0.9727 \pm 0.0044 } $ &            $  \underline{ 0.9724 \pm 0.0045 } $ \\
       & ind-RNNSig &                           $ 0.9975 \pm 0.00028 $ &                           $ 0.9349 \pm 0.0062 $ &                           $ 0.9341 \pm 0.0061 $ \\
       & ind-Sig &                           $ 0.9941 \pm 0.00031 $ &                           $ 0.9059 \pm 0.0031 $ &                           $ 0.9049 \pm 0.0031 $ \\
       & lin-DeepSig &                           $ 0.9946 \pm 0.00052 $ &                           $ 0.9157 \pm 0.0041 $ &                           $ 0.9145 \pm 0.0042 $ \\
       & lin-RNN &                           $ 0.9949 \pm 0.00093 $ &                           $ 0.9161 \pm 0.0061 $ &                           $ 0.9149 \pm 0.0061 $ \\
       & lin-RNNSig &                           $ 0.9945 \pm 0.00039 $ &                           $ 0.9026 \pm 0.0086 $ &                           $ 0.9014 \pm 0.0087 $ \\
       & lin-Sig &                           $ 0.9896 \pm 0.00084 $ &                           $ 0.8725 \pm 0.0044 $ &                           $ 0.8714 \pm 0.0046 $ \\
       & zero-DeepSig &                           $ 0.9939 \pm 0.00071 $ &                           $ 0.9112 \pm 0.0041 $ &                            $ 0.9101 \pm 0.004 $ \\
       & zero-RNN &                           $ 0.9955 \pm 0.00031 $ &                           $ 0.9177 \pm 0.0028 $ &                            $ 0.9167 \pm 0.003 $ \\
       & zero-RNNSig &                           $ 0.9932 \pm 0.00033 $ &                           $ 0.8954 \pm 0.0041 $ &                           $ 0.8946 \pm 0.0042 $ \\
       & zero-Sig &                           $ 0.9854 \pm 0.00069 $ &                           $ 0.8427 \pm 0.0044 $ &                           $ 0.8419 \pm 0.0045 $ \\
Random & GP-DeepSig &                            $ 0.9051 \pm 0.0016 $ &                           $ 0.5454 \pm 0.0043 $ &                           $ 0.5451 \pm 0.0045 $ \\
       & GP-RNN &                            $ 0.9196 \pm 0.0086 $ &                            $ 0.5793 \pm 0.021 $ &                             $ 0.579 \pm 0.021 $ \\
       & GP-RNNSig &                            $ 0.8674 \pm 0.0059 $ &                            $ 0.4684 \pm 0.013 $ &                            $ 0.4687 \pm 0.012 $ \\
       & GP-Sig &                            $ 0.8351 \pm 0.0049 $ &                           $ 0.4175 \pm 0.0043 $ &                           $ 0.4181 \pm 0.0042 $ \\
       & GP-PoM-DeepSig &                           $ 0.9951 \pm 0.00078 $ &                           $ 0.9215 \pm 0.0056 $ &                            $ 0.921 \pm 0.0055 $ \\
       & GP-PoM-RNN &                           $ 0.9956 \pm 0.00072 $ &            $  \underline{ 0.9276 \pm 0.0074 } $ &             $  \underline{ 0.927 \pm 0.0073 } $ \\
       & GP-PoM-RNNSig &                            $ 0.9897 \pm 0.0025 $ &                            $ 0.8815 \pm 0.016 $ &                            $ 0.8811 \pm 0.016 $ \\
       & GP-PoM-Sig &                           $ 0.9903 \pm 0.00099 $ &                            $ 0.8735 \pm 0.009 $ &                            $ 0.8729 \pm 0.009 $ \\
       & causal-DeepSig &                             $ 0.991 \pm 0.0012 $ &                           $ 0.8948 \pm 0.0036 $ &                           $ 0.8943 \pm 0.0036 $ \\
       & causal-RNN &                           $ 0.9929 \pm 0.00066 $ &                           $ 0.8953 \pm 0.0054 $ &                           $ 0.8947 \pm 0.0054 $ \\
       & causal-RNNSig &                           $ 0.9917 \pm 0.00067 $ &                           $ 0.8881 \pm 0.0061 $ &                           $ 0.8876 \pm 0.0062 $ \\
       & causal-Sig &                            $ 0.9787 \pm 0.0022 $ &                           $ 0.8007 \pm 0.0098 $ &                           $ 0.8001 \pm 0.0097 $ \\
       & ff-DeepSig &                           $ 0.9914 \pm 0.00068 $ &                           $ 0.8897 \pm 0.0066 $ &                            $ 0.889 \pm 0.0064 $ \\
       & ff-RNN &                           $ 0.9931 \pm 0.00067 $ &                           $ 0.9007 \pm 0.0025 $ &                           $ 0.9003 \pm 0.0025 $ \\
       & ff-RNNSig &                            $ 0.992 \pm 0.00063 $ &                           $ 0.8893 \pm 0.0051 $ &                            $ 0.889 \pm 0.0053 $ \\
       & ff-Sig &                           $ 0.9843 \pm 0.00069 $ &                           $ 0.8446 \pm 0.0047 $ &                           $ 0.8437 \pm 0.0048 $ \\
       & ind-DeepSig &               $  \mathbf{ 0.9961 \pm 0.00059 } $ &               $  \mathbf{ 0.9316 \pm 0.0074 } $ &               $  \mathbf{ 0.9309 \pm 0.0075 } $ \\
       & ind-RNN &  $  \mathbf{ \underline{ 0.9973 \pm 0.00044 }} $ &  $  \mathbf{ \underline{ 0.9412 \pm 0.0041 }} $ &  $  \mathbf{ \underline{ 0.9407 \pm 0.0041 }} $ \\
       & ind-RNNSig &                           $ 0.9955 \pm 0.00041 $ &                            $ 0.916 \pm 0.0028 $ &                           $ 0.9153 \pm 0.0027 $ \\
       & ind-Sig &                            $ 0.9871 \pm 0.0004 $ &                           $ 0.8454 \pm 0.0054 $ &                           $ 0.8451 \pm 0.0056 $ \\
       & lin-DeepSig &                            $ 0.9941 \pm 0.0015 $ &                            $ 0.9142 \pm 0.011 $ &                            $ 0.9137 \pm 0.011 $ \\
       & lin-RNN &                           $ 0.9951 \pm 0.00041 $ &                           $ 0.9186 \pm 0.0058 $ &                           $ 0.9181 \pm 0.0059 $ \\
       & lin-RNNSig &            $  \underline{ 0.9959 \pm 0.00036 } $ &                           $ 0.9156 \pm 0.0052 $ &                           $ 0.9152 \pm 0.0054 $ \\
       & lin-Sig &                           $ 0.9903 \pm 0.00094 $ &                           $ 0.8712 \pm 0.0061 $ &                           $ 0.8704 \pm 0.0061 $ \\
       & zero-DeepSig &                           $ 0.9933 \pm 0.00077 $ &                           $ 0.8977 \pm 0.0054 $ &                           $ 0.8969 \pm 0.0055 $ \\
       & zero-RNN &                             $ 0.994 \pm 0.0011 $ &                           $ 0.9073 \pm 0.0062 $ &                            $ 0.907 \pm 0.0062 $ \\
       & zero-RNNSig &                           $ 0.9915 \pm 0.00046 $ &                           $ 0.8795 \pm 0.0025 $ &                           $ 0.8788 \pm 0.0024 $ \\
       & zero-Sig &                           $ 0.9862 \pm 0.00073 $ &                           $ 0.8393 \pm 0.0038 $ &                           $ 0.8391 \pm 0.0037 $ \\
\bottomrule
\end{tabular}

